Policy Optimization with Stochastic Mirror Descent

Improving sample efficiency has been a longstanding goal in reinforcement learning. This paper proposes $\mathtt{VRMPO}$ algorithm: a sample efficient policy gradient method with stochastic mirror descent. In $\mathtt{VRMPO}$, a novel variance-reduced policy gradient estimator is presented to improve sample efficiency. We prove that the proposed $\mathtt{VRMPO}$ needs only $\mathcal{O}(\epsilon^{-3})$ sample trajectories to achieve an $\epsilon$-approximate first-order stationary point, which matches the best sample complexity for policy optimization. The extensive experimental results demonstrate that $\mathtt{VRMPO}$ outperforms the state-of-the-art policy gradient methods in various settings.

==> abstract.tex <==
%!TEX root = main.tex
We focus on using Thompson Sampling to solve unimodal bandit problems, where the expected reward is monotonic over the partially ordered arms.
Although \cite{paladino2017unimodal,trinh2020solving} have extended Thompson Sampling to unimodal multi-armed bandits, 
their methods heavily depend on a \emph{forced-exploitation} mechanism that forces the player to pull the current leader (i.e., the action maintains the maximal empirical mean of rewards) at a fixed frequency.
Forced-exploitation separates exploration from exploitation rounds, which is undesirable for multi-armed bandit problems.
Additionally,
tuning the frequency factor manually for the forced-exploitation method is inefficient for complex sequence decision-making tasks, 
and it is still a debate that whether or not those forcing mechanisms are desirable for unimodal bandits.



To address the above problems, we propose the $\texttt{FEF}$-$\texttt{UTS}$ (forced-exploitation free unimodal Thompson Sampling) algorithm.
The proposed $\texttt{FEF}$-$\texttt{UTS}$ does not consider the forced-exploitation mechanism, i.e.,
$\texttt{FEF}$-$\texttt{UTS}$ does not force the player to pull the current leader.
To exploit the unimodal structure better, 
at each step, instead of exploration from the entire decision space,
$\texttt{FEF}$-$\texttt{UTS}$ makes decisions only in the neighborhood of the arm that has the highest empirical mean reward.
We theoretically prove that, for Bernoulli rewards, the upper bound regret of $\texttt{FEF}$-$\texttt{UTS}$ matches the lower asymptotic bound regret of unimodal bandits, thus $\texttt{FEF}$-$\texttt{UTS}$ is an asymptotically optimal algorithm. 
Finally, we use experiments to demonstrate the effectiveness of the proposed algorithm, results show that $\texttt{FEF}$-$\texttt{UTS}$ performs better than extensive state-of-the-art algorithms.
We have opened our code at: \url{https://github.com/jijiaming-bit/FEF-UTS}.

==> app_preliminary.tex <==
\section{Notation}


For convenience of reference, we list key notations that have be used in this paper.


\begin{tabular}{r c p{13cm}}
        $[K]$ &: & The space of actions: $[K]=\{1,2,\cdots,K\}$. \\
	$T$ &: & The horizon. \\
	$a_{t}$ &:& The action (the arm be played) in round $t$.\\
	$\nu_{a}$ & : & The unknown (but fixed) reward distribution of arm $a$\\
	$\mu_{a}$ &:& The expectation of value of arm $a$.\\
	$\mu^{\star}$ &:& The maximum expectation of value, i.e., $\mu^{\star}=\max_{a\in[K]}\mu_a$.\\
	$a^{\star}$ &:& The optimal action that satisfies $a^{\star}=\arg\max_{a\in[K]}\{\mu_{a}\}$.\\
	$\Delta_a$ & : & The gap between the mean of the optimal arm and the mean of arm $a$, $\Delta_a = \mu^{\star}-\mu_a$.\\
	$\delta_{a}(x)$ & : & $\delta_{a}(x)=\mu_a-x$.\\
	$D_a(x)$ & : & $D_a(x)=\mathbb{KL}(x|\mu_a)$ is KL-divergence between Bernoulli distributions with parameters $\mu_a$ and $x$.\\
	$X_{a,t}$& : & The reward after playing $a$ at time $t$.\\
	$\mathcal{G}$& : & The undirected graph.	\\
         $\mathcal{V}$& : & The set of vertices of the undirected graph $\mathcal{G}$.\\
	$\mathcal{E}$& : & The set of edges of the undirected graph $\mathcal{G}$.\\
	$\nu$& : & The joint reward distribution $\nu=(\nu_{1},\cdots,\nu_{K})$.\\
	 $\mathcal{N}(i)$ & : &The neighborhood of arm $i$: $\mathcal{N}(i)=\{j|(i,j)\in\mathcal{E}\}$.\\
	 $\mathcal{N}^{+}({i})$ & : &The extended neighborhood of arm $i$: $\mathcal{N}^{+}(i)=\mathcal{N}(i)\cup\{i\}$.\\
	  %$\mathcal{N}(\mu,\sigma^2)$ & : &The Gaussian distribution with mean value $\mu$ and variance $\sigma^2$.\\
	  $\mathcal{B}(\mu)$ & : &Bernoulli distribution with expectation $\mu$.\\
	 $N_{a,t}$& : & The number of times that arm $a$ has been chosen at the end of round $t$: $N_{a,t}=\sum_{s=1}^{t}\mathbb{I}\{{a_s=a}\}$.\\
	  $L_{t}$& : & The leader at round $t$.\\
	 $n_{a,t}$& : & The number of times arm $a$ has been chosen as a leader at the end of round $t$.\\
	 $\hat{\mu}_a (n)$& : &  $\hat{\mu}_a (n)$ denotes the empirical mean reward of arm $a$ with $n$ samples. \\
	 $\hat{\mu}_{a,t}$ & : &  $\hat{\mu}_{a,t}$ denotes the empirical reward of the arm $a$ at round $t$. 
\end{tabular}






\clearpage
\section{Auxiliary Results}



\subsection{Chernoff-Hoeffding Bound}

\begin{fact}[Chernoff-Hoeffding Bound] 
\label{fact:chernoff-hoeffding-01}
Let $X_{1},\cdots,X_n$ be independent Bernoulli random variables with $\mathbb{E}[X_i]=p_i$, let $X=\frac{1}{n}\sum_{i=1}^{n}X_i$, $\mu=\frac{1}{n}\sum_{i=1}^{n}p_i$, then for any $\lambda\in(0,1-\mu)$, 
\[
\mathbb{P}(X\ge\mu+\lambda)\leq\exp{\left\{-n\mathbb{KL}(\mu+\lambda|\mu)\right\}};
\]
and for any $\lambda\in(0,\mu)$,
\[
\mathbb{P}(X\leq\mu-\lambda)\leq\exp{\left\{-n\mathbb{KL}(\mu-\lambda|\mu)\right\}}.
\]
\end{fact}
We omit its proof, e.g., \citep[Chapter 10]{lattimore2018bandit} provide a proof.




\subsection{Relationship between Beta Distribution and Binomial Distribution}
\label{sec:bb-relation}


Let $F^{\text{Beta}}_{a,b}$ denote the c.d.f of a Beta distribution with parameters $a$ and $b$, $F^{\text{B}}_{n,p}(k)$ denotes the c.d.f of a Binomial distribution with parameters $n$ and $p$, i.e., 
\[ F^{\text{Beta}}_{a,b}(x)=\frac{\Gamma(a+b)}{\Gamma(a)\Gamma(b)}\int_{0}^{x}\xi^{a-1}(1-\xi)^{b-1}\text{d}\xi,~~~~F^{\text{B}}_{n,p}(k)=(n-k){n \choose k}\int _{0}^{1-p}\xi^{n-k-1}(1-\xi)^{k}\,\text{d}\xi,\]
where \[\Gamma(x)=\int_{0}^{+\infty}\xi^{x-1}e^{-\xi}\text{d}\xi\] is the Gamma function. Then, we have 
\begin{flalign}
\label{cdf-beta-binomial}
F^{\text{Beta}}_{a,b}(y)=1-F^{\text{B}}_{a+b-1,y}(a-1).
\end{flalign}



Finally, we introduce a notation $\Theta(\cdot)$. For any two functions $f(n),g(n)$, \[f(n) = \Theta(g(n))\] if there exist constants $b,c$ and $n_0$ such that for all $n \ge n_0$, $bg(n) \ge f(n) \ge cg(n).$


\begin{lemma}
[Lemma 2 in \cite{agrawal2013further}]
\label{app-lemma-bound-pka}
Let $a\in[K]$, $n\ge 0$ and $0<x <\mu_{a}$.
Let $\hat{\mu}_{a}(n)$ be the empirical average of $n$ samples from the Bernoulli distribution with expectation $\mu_a$. 
Let \[p_{a,n}(x)=1-F^{\emph{Beta}}_{(n+1)\hat{\mu}_{a}(n),(n+1)(1-\hat{\mu}_{a}(n))}(x)\] be the probability that the posterior sample from the Beta distribution with its parameter
$(n+1)\hat{\mu}_{a}(n),(n+1)(1-\hat{\mu}_{a}(n))$ exceeds $x$, where $\hat{\mu}_a (n)$ denotes the empirical mean reward of arm $a$ with $n$ samples. Then, its average over runs is bounded as
$$ \mathbb{E}\left[\dfrac{1}{p_{a,n}(x)}-1\right]=\left\{
\begin{array}{rcl}
&\dfrac{3}{\delta_{a}(x)},      & {n<\dfrac{8}{\delta_{a}(x)} }\\\\
&\Theta 
\left(
e^{-\frac{1}{2}n\delta^{2}_{a}(x)}+\dfrac{e^{-n D_{a}(x)}}{(n+1)\delta^{2}_{a}(x)}+\dfrac{1}{e^{\frac{n}{4}\delta^{2}_{a}(x)}-1}
 \right)                  
 & {n\ge\dfrac{8}{\delta_{a}(x)},}
\end{array} \right. $$
where $\delta_{a}(x)=\mu_a-x$, $D_a(x)=\mathbb{KL}(x|\mu_a)$ is KL-divergence between Bernoulli distributions with parameters $\mu_a$ and $x$.
\end{lemma}





\section{Proof of Theorem \ref{}}









\begin{lemma}
\label{lemma-5}
Recall $n_{a,t}$ denotes the number of times arm $a$ has been chosen as the leader at the end of round $t$, then 
regret $R_{2}(T)$ is upper-bounded as follows,
\begin{flalign}
\label{app-upp-r-2}
R_{2}(T)\leq
\sum_{a\ne a^\star}\mathbb{E}[n_{a,T}].
\end{flalign}
\end{lemma}
\begin{proof}
The result (\ref{app-upp-r-2}) has appeared in \cite{combes2014unimodal_a,paladino2017unimodal,trinh2020solving}.
For completeness, we use our notations to present it as follows:
\begin{flalign}
\label{app-r2-01}
R_2(T)&=\sum_{a\ne a^\star}\underbrace{(\mu^{\star}-\mu_a)}_{\leq 1}\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{L_{t}\ne a^\star,a_t=a\}
\right ]
\leq\sum_{a\ne a^\star}\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{L_{t}\ne a^\star,a_t=a\}\right ].
\end{flalign}
Furthermore, the following events occur
\[
\{L_{t}\ne a^\star,a_t=a\}
\subset
\{L_{t}\ne a^\star\}=\{L_{t}=\tilde a, \tilde{a}\ne a^{\star}\},
\]
which implies 
\[
\mathbb{I}
\{L_{t}\ne a^\star,a_t=a\}
\leq
\mathbb{I}
\{L_{t}=\tilde a, \tilde{a}\ne a^{\star}\}.
\]
Sum it up on the space $[K]-\{a^{\star}\}$, we have
\begin{flalign}
\nonumber
\sum_{a\ne a^\star}\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{L_{t}\ne a^\star,a_t=a\}\right ]
\leq&
\sum_{\tilde{a}\ne a^\star}\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{L_{t}=\tilde a, \tilde{a}\ne a^{\star}\}\right ]
\\
\nonumber
=&\sum_{a\ne a^\star}\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{L_{t}=a\ne a^{\star}\}\right ]
=\sum_{a\ne a^\star}\mathbb{E}[n_{a,T}],
\end{flalign}
recall the result (\ref{app-r2-01}), we achieve $R_{2}(T)\leq
\sum_{a\ne a^\star}\mathbb{E}[n_{a,T}]$.


This concludes the proof of Lemma \ref{lemma-5}.
\end{proof}


\begin{lemma}
\label{app:lemma5-01}
The term $\sum_{a\ne a^\star}\mathbb{E}[n_{a,T}]$ is upper bounded as follows:
\begin{flalign}
\label{app:lemma5-02}
\sum_{a\ne a^\star}\mathbb{E}[n_{a,T}]\leq\underbrace{\sum_{a\ne a^\star}\sum_{t=1}^{T}\mathbb{P}\left(\hat{\mu}_{a,t}-\mu_a\ge \dfrac{\Delta_a}{2}\right)}_{\emph{Term~I}}
+\underbrace{\sum_{a\ne a^\star}\sum_{t=1}^{T}\mathbb{P}\left(\mu^\star- \hat{\mu}_{a^\star,t}\ge\frac{\Delta_a}{2}\right)}_{\emph{Term~II}}.
\end{flalign}
\end{lemma}





\begin{proof}
According to the definition of the leader: $L_t=\arg\max_{a\in [K]}\{\hat{\mu}_{a,t}\}$, if $L_t =a$, we have 
\begin{flalign}
\nonumber
\sum_{a\ne a^\star}\mathbb{E}[n_{a,T}]&=:
\sum_{a\ne a^\star}\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{L_{t}=a\}\right]\\
\label{app-a-7}
&=\sum_{a\ne a^\star}\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\left\{\hat{\mu}_{a,t}=\max_{i\in[K]}\hat{\mu}_{i,t}\right\}\right]=\sum_{a\ne a^\star}\sum_{t=1}^{T}\mathbb{P}\left(\hat{\mu}_{a,t}=\max_{i\in[K]}\hat{\mu}_{i,t}\right).
\end{flalign}
Since we consider the case $L_t=a\ne a^\star$, i.e., the case that the suboptimal arm $a$  selected as a leader, then 
\[\hat{\mu}_{a,t}\ge\hat{\mu}_{a^\star,t}.\]
It is easy to check that $\{\hat{\mu}_{a,t}=\max_{i\in[K]}\hat{\mu}_{i,t}\}\subset\{\hat{\mu}_{a,t}\ge\hat{\mu}_{a^\star,t}\}$, which implies 
\begin{flalign}
\label{app-a-7-1}
\mathbb{P}\left(\hat{\mu}_{a,t}=\max_{i\in[K]}\hat{\mu}_{i,t}\right)\leq\mathbb{P}(\hat{\mu}_{a,t}\ge\hat{\mu}_{a^\star,t}).
\end{flalign}
Recall $\Delta_{a}=\mu^\star-\mu_a$, $a\in [K]$,  
thus, we have
\begin{flalign}
%\label{app-a-8}
\nonumber
\sum_{a\ne a^\star}\mathbb{E}[n_{a,T}]&\overset{(\ref{app-a-7})}=\sum_{a\ne a^\star}\sum_{t=1}^{T}\mathbb{P}\left(\hat{\mu}_{a,t}=\max_{i\in[K]}\hat{\mu}_{i,t}\right)\\
\label{app-a-9}
&\overset{(\ref{app-a-7-1})}\leq \sum_{a\ne a^\star}\sum_{t=1}^{T}\mathbb{P}(\hat{\mu}_{a,t}\ge\hat{\mu}_{a^\star,t})\\
%\label{app-a-10}
\nonumber
&= \sum_{a\ne a^\star}\sum_{t=1}^{T}\mathbb{P}\left(\hat{\mu}_{a,t}-\mu_a-\frac{\Delta_a}{2}+\mu^\star- \hat{\mu}_{a^\star,t}-\frac{\Delta_a}{2}\ge0\right)\\
%\label{app-a-11}
\nonumber
&\leq \sum_{a\ne a^\star}\sum_{t=1}^{T}\left[\mathbb{P}\left(\hat{\mu}_{a,t}-\mu_a-\frac{\Delta_a}{2}\ge 0\right)+\mathbb{P}\left(\mu^\star- \hat{\mu}_{a^\star,t}-\frac{\Delta_a}{2}\ge0\right)\right]\\
\label{app-a-12}
&= \sum_{a\ne a^\star}\sum_{t=1}^{T}\left[\mathbb{P}\left(\hat{\mu}_{a,t}-\mu_a\ge \dfrac{\Delta_a}{2}\right)+\mathbb{P}\left(\mu^\star- \hat{\mu}_{a^\star,t}\ge\frac{\Delta_a}{2}\right)\right].
\end{flalign}

This concludes the proof of Lemma \ref{app:lemma5-01}.
\end{proof}










==> mab.tex <==
\chapter{Stochastic Multi-arms Bandits}
\label{chap:s-mab}


We consider the MAB (stochastic multi-armed bandit) with $K$ arms.
At each round $t\in\mathbb{N}$, the decision maker pulls an arm $a\in[K]=:\{1,2,\cdots,K\}$, 
then it receives a random reward $X_{a,t}$ according to an unknown (but fixed) distribution $\nu_{a}$ that has an expectation $\mu_{a}=\mathbb{E}[X_{a,t}]$.
The random reward of each arm is independent identically distributed, 
and it is independent of the plays of other arms.
We assume that there is a unique optimal arm $a^{\star}$ satisfies 
\[\mu^{\star}=:\max_{a\in[K]}\mu_{a},~~~a^{\star}=\arg\max_{a^{'}\in[K]}\mu_{a^{'}}.\]
We use $\Delta_a =: \mu^{\star}-\mu_a$ to denote the gap between the mean of the arm $a^{\star}$ and arm $a$.


For the standard MAB problem, we use the loss of all generated rewards to measure the performance of a policy $\pi$.
Let $\mathcal{A}=\{ a_{t}\}_{t=1}^{T}$ be an action sequence that is generated by $\pi$.
The regret of the policy $\pi$ is defined as 
\[R^{\pi}(T)=\mathbb{E}\left[\sum_{t=1}^{T}(\mu^{\star}-X_{a_t,t})\right],\]
where the expectation $\mathbb{E}[\cdot]$ is taken with respect to the measure on outcomes induced by the interaction of the policy $\pi$ and the joint reward distribution $\nu$.
Let \[N_{a,t}=\sum_{j=1}^{t}\mathbb{I}\{{a_j=a}\}\] be the number of times arm $a$ has been played after $t$ rounds, where $\mathbb{I}\{\cdot\}$ is the indicator function, i.e., $\mathbb{I}\{{E}\}=1$ if ${E}$ occurs; otherwise $\mathbb{I}\{{E}\}=0$.
Then the regret can be written as follows,
\begin{flalign}
R^{\pi}(T)=\sum_{a\in[K]}\Delta_a \mathbb{E}[N_{a,T}].
\end{flalign}


Let 
\[\hat{\mu}_{a,t}=\dfrac{\sum_{j=1}^{t}\mathbb{I}\{{a_j=a}\}X_{a,j}}{N_{a,t}},~~~a\in[K]
\]
be the empirical reward mean received from arm $a$ at round $t$ and current best mean.








\section{Upper Confidence Bound (UCB) Algorithms}
\label{chap:s-mab-sub-01}


\subsection{UCB1 \citep{auer2002finite}}


\begin{proposition}[\citep{hoeffding1963probability}]
\label{prop:hoeffding1963probability-eq}
Let $X_1,\cdots, X_n$ be independent random variables bounded by the interval $[0, 1]: 0 \leq X_i \leq1$, and $\E[X_i]=\mu$.
We define the empirical mean of these variables by $\hat{\mu}_{n}=\frac{1}{n}(X_1+X_2+\cdots+X_n),$ then for any $\epsilon>0$
\begin{flalign}
\label{app-a-lemma}
\mathbb{P} (|\hat{\mu}_{n}-\mu|\geq \epsilon)\leq \exp\{-2n\epsilon^{2}\}.
\end{flalign}
\end{proposition}

Furthermore, Proposition \ref{prop:hoeffding1963probability-eq} implies for any $\delta\in(0,1)$, the following holds with probability at least $1-\delta$, 
\begin{flalign}
\mu\leq \hat{\mu}_{n}+\sqrt{\dfrac{1}{2n}\log\frac{1}{\delta}},~~~~\mu\ge \hat{\mu}_{n}-\sqrt{\dfrac{1}{2n}\log\frac{1}{\delta}}.
\end{flalign}

Firstly, we state a version of UCB in Algorithm \ref{algo: ucb1}.
Let’s explain why UCB-based rule makes sense. 
When the player pulls an arm $a$ at round $t$, the arm $a$ keeps the maximal $\mathtt{UCB}_{a,t}$, where
$
\mathtt{UCB}_{a,t}=
\hat{\mu}_{a,t}+c_{a,t},~c_{a,t}=\sqrt{\dfrac{\alpha \log t}{N_{a,t}}}.
$
That happens due to two facts: 
\begin{itemize}
\item $\hat{\mu}_{a,t}$ is larger, for which the arm $a$ is likely to have a high reward;
\item otherwise the confidence radius $c_{a,t}$ is larger, for which the arm $a$ has not been explored much.
\end{itemize}
Either reason makes this arm $a$ worth to be pulled.
Furthermore, the values $\hat{\mu}_{a,t}$ and $c_{a,t}$ summand in the UCB represent exploitation and exploration, respectively, and summing them up is a natural way to trade off the two.

\begin{algorithm}[t]
\caption{$\mathtt{UCB1}$ \citep{auer2002finite}}
\label{algo: ucb1}
\begin{algorithmic}[1]
\STATE Play each arm once, $t\leftarrow K$;
\FOR{$t=K,\cdots , T$}
\STATE Play $a_t=\arg\max_{a\in[K]}\left(\hat{\mu}_{a,t}+\sqrt{\dfrac{\alpha \log t}{N_{a,t}}}\right)$
\ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{theorem}[Regret Analysis of $\mathtt{UCB1}$]
\label{theo:regret-of-ucb1}
Assume the reward is in $[0,1]$, $\alpha>1$, then the regret of $\mathtt{UCB1}$ (Algorithm \ref{algo: ucb1}) is upper-bounded as follows
\[
R^{\mathtt{UCB1} }(T)\leq
\sum_{a\ne a^{\star}}
\left(
\dfrac{4\alpha \log T}{\Delta_a}+c\Delta_a
\right),
\]
where $c>0$.
\end{theorem}

\begin{proof}
To simplify the proof, we assume the reward is in $[0,1]$, and we ignore the initial exploration since the regret of initial exploration is at most $K$.
Let 
\begin{flalign}
\label{three-events}
\mathcal{A}_{a^{\star},t}=\left\{
\hat{\mu}_{a^{\star},t}+\sqrt{\dfrac{\alpha \log t}{N_{a^{\star},t}}}\leq\mu^{\star}
\right\},
\mathcal{B}_{a,t}=\left\{
{\mu}_{a}+\sqrt{\dfrac{\alpha \log t}{N_{a,t}}}<\hat{\mu}_{a,t}
\right\},
\mathcal{C}_{a,t}=\left\{
N_{a,t}\leq \dfrac{4\alpha \log t}{\Delta_a^2}
\right\},
\end{flalign}
where $a\in[K]$.
$\mathcal{A}_{a^{\star},t}$ denotes underestimation of optimal arm $a^{\star}$, $\mathcal{B}_{a,t}$ denotes overestimation of suboptimal arm $a$, and $\mathcal{C}_{a,t}$ denotes that arm $a$ is not sufficiently sampled.


Firstly, we note that if $a_t=a\in [K]$,
then at least one of the three events $\mathcal{A}_{a^{\star},t},\mathcal{B}_{a,t},\mathcal{C}_{a,t}$ should occur.
In fact, if none of those events occur, i.e., all above three events are all false, then we have
\begin{flalign}
\hat{\mu}_{a^{\star},t}+\sqrt{\dfrac{\alpha \log t}{N_{a^{\star},t}}}>\mu^{\star}=\mu_a+\Delta_a>\mu_a+2\sqrt{\dfrac{\alpha \log t}{N_{a,t}}}\ge \hat{\mu}_k+\sqrt{\dfrac{\alpha \log t}{N_{a,t}}},
\end{flalign}
which is a contradiction with the fact $a_t=a$.
Thus, we have
\begin{flalign}
\label{decompose-a-t}
\{a_t=a\}\subset\mathcal{A}_{a^{\star},t}\cup\mathcal{B}_{a,t}\cup\mathcal{C}_{a,t}.
\end{flalign}



Since 
\[\left\{\hat{\mu}_{a^{\star},t}+\sqrt{\dfrac{\alpha \log t}{N_{a^{\star},t}}}\leq\mu^{\star},N_{a^{\star},t}=i\right\}\bigcap\left\{\hat{\mu}_{a^{\star},t}+\sqrt{\dfrac{\alpha \log t}{N_{a^{\star},t}}}\leq\mu^{\star},N_{a^{\star},t}=j\right\}=\varnothing, i\ne j,\] 
then the event $ \mathcal{A}_{a^{\star},t}$ can decomposed as follows,
\[
 \mathcal{A}_{a^{\star},t}=
\bigcup_{n=1}^{t}
\left\{\hat{\mu}_{a^{\star},t}+\sqrt{\dfrac{\alpha \log t}{N_{a^{\star},t}}}\leq\mu^{\star},N_{a^{\star},t}=n\right\}.
\]
Furthermore, if $\alpha>1$,
we have
\begin{flalign}
\nonumber
 \sum_{t=1}^{T}\mathbb{P}
 \left[
 \mathcal{A}_{a^{\star},t}
   \right]
 \leq&\sum_{t=1}^{T}\sum_{n=1}^{t}\mathbb{P}
 \left[
\hat{\mu}_{a^{\star},t}+\sqrt{\dfrac{\alpha \log t}{N_{a^{\star},t}}}\leq\mu^{\star},N_{a^{\star},t}=n
 \right]\\
 \nonumber
 =&\sum_{t=1}^{T}\sum_{n=1}^{t}\mathbb{P}
 \left[
\hat{\mu}_{a^{\star},t}+\sqrt{\dfrac{\alpha \log t}{n}}\leq\mu^{\star}
 \right]
 =\sum_{t=1}^{T}\sum_{n=1}^{t}\dfrac{1}{t^{2\alpha}}=\sum_{t=1}^{T}\dfrac{1}{t^{2\alpha-1}}\leq+\infty.
\end{flalign}
The same upper bound holds for the event $\mathcal{B}_{a,t}$.
\begin{flalign}
\sum_{t=1}^{T}\mathbb{I}\{\mathcal{C}_{a,t}\}\leq \dfrac{4\alpha \log T}{\Delta_a}+\mathbb{I}\left\{\mathcal{C}_{a,t},{N}_{a,t}> \dfrac{4\alpha \log T}{\Delta_a}\right\}=\dfrac{4\alpha \log T}{\Delta_a^2}.
\end{flalign}
Finally, recall the result (\ref{decompose-a-t}), then there exists a positive scalar $c$ such that
\begin{flalign}
\mathbb{E}[{N_{a,T}}]=\E\left[\sum_{t=1}^{T}\I\{{a_t=a}\}\right]=\sum_{t=1}^{T}\P\{{a_t=a}\}\leq \sum_{t=1}^{T}\left( \P[\mathcal{A}_{a^{\star},t}]+\P[\mathcal{B}_{a,t}]+\P[\mathcal{C}_{a,t}]\right)\leq \dfrac{4\alpha \log T}{\Delta_a}+c.
\end{flalign}

This concludes the proof.
\end{proof}


\begin{remark}
It is a natural question: 
\begin{center}
what inspires us to construct the three events $\calA_{a^{\star},t},\calB_{a,t},\calC_{a,t}$ (\ref{three-events})?
\end{center}
In this section, we provide a derivation of a special case $\alpha=2$.
Let us go back to the analysis of \cite{auer2002finite}.
Let $\ell$ be any positive integer, and $c_{a,t}=\sqrt{\dfrac{2\log t}{N_{a,t}}}$, then
\begin{flalign}
\nonumber
N_{a,T}=&1+\sum_{t=K+1}^{T}\I\{a_t=a\}\\
\nonumber
\leq&\ell+\sum_{t=K+1}^{T}\I
\left\{
a_t=a,N_{a,{t-1}}\ge \ell
\right\}
\\
\nonumber
\leq&\ell+\sum_{t=K+1}^{T}\I
\left\{
\hat{\mu}_{a^{\star},t-1}+c_{a^{\star},t-1}\leq\hat{\mu}_{a,t-1}+c_{a,t-1}
,N_{a,{t-1}}\ge \ell
\right\}
\tag*{$\blacktriangleright$ Playing $a_t=a$}
\\
\label{chap:s-mab-sub-01-01}
\leq&\ell+\sum_{t=K+1}^{T}\I
\left\{
\min_{0<i<t}
\left \{
\hat{\mu}_{a^{\star},i}+c_{a^{\star},i}
 \right\}
\leq
\max_{\ell<j<t}
\hat{\mu}_{a,j}+c_{a,j}
\right\}
\\
\label{chap:s-mab-sub-01-02}
\leq&\ell+\sum_{t=K+1}^{T}
\sum_{i=1}^{t-1}
\sum_{j=\ell}^{t-1}
\I
\left\{
\hat{\mu}_{a^{\star},i}+c_{a^{\star},i}
\leq
\hat{\mu}_{a,j}+c_{a,j}
\right\},
\end{flalign}
where (\ref{chap:s-mab-sub-01-01}) holds since we do by contradiction as follows; the event 
\[\left\{
\min_{0<i<t}
\left \{
\hat{\mu}_{a^{\star},i}+c_{a^{\star},i}
 \right\}
>
\max_{\ell<j<t}
\hat{\mu}_{a,j}+c_{a,j}
\right\}\]
is a contradiction with the fact that $a_t=a$, if $N_{a,{t-1}}\ge \ell$;
(\ref{chap:s-mab-sub-01-01}) holds since 
\[
\left\{
\min_{0<i<t}
\left \{
\hat{\mu}_{a^{\star},i}+c_{a^{\star},i}
 \right\}
\leq
\max_{\ell<j<t}
\hat{\mu}_{a,j}+c_{a,j}
\right\}=
\bigcup_{i=1}^{t-1}\bigcup_{j=\ell}^{t-1}\left\{
\hat{\mu}_{a^{\star},i}+c_{a^{\star},i}
\leq
\hat{\mu}_{a,j}+c_{a,j}
\right\}.
\]
Furthermore, $\hat{\mu}_{a^{\star},i}+c_{a^{\star},i}\leq\hat{\mu}_{a,j}+c_{a,j}$ implies that at least one of the following three events must hold
\begin{flalign}
\label{chap:s-mab-sub-01-03}
\hat{\mu}_{a^{\star},i}\leq\mu^{\star}-c_{a^{\star},i},~~
\hat{\mu}_{a,j}\ge\mu_a+c_{a,j},~~\mu^{\star}<\mu_a+2c_{a,j}.
\end{flalign}
Finally, let $\mu^{\star}<\mu_a+2c_{a,j}$ hold, we have
\begin{flalign}
\label{chap:s-mab-sub-01-04}
N_{a,t}\leq \dfrac{8 \log t}{\Delta_a^2}.
\end{flalign}
The results (\ref{chap:s-mab-sub-01-03})-(\ref{chap:s-mab-sub-01-04}) are the original idea of the construction of three events (\ref{three-events}).
\end{remark}


This proof of Theorem \ref{theo:regret-of-ucb1} is adaptive to Theorem 2.1 of \citep{bubeck2012regret}, where they they extend the distribution of rewards $X$ satisfies the following moment conditions: there exists a convex function $\psi(\cdot)$ such that, for all $\lambda>0$,
\begin{flalign}
\label{def:sub-gauassian}
\log \E \left[e^{\lambda(X-\E [X])}\right]\leq \psi(\lambda),~~\log \E \left[e^{\lambda(\E [X]-X)}\right]\leq \psi(\lambda).
\end{flalign}
Furthermore, using Markov's inequality, we have
\begin{flalign}
\label{concention-ineq-01}
\P
\left[
\mu_a -\hat{\mu}_{a,t}>\epsilon
\right]
\leq \exp\left\{-N_{a,t}\psi^{\star}(\epsilon)\right\},
\end{flalign}
where $\psi^{\star}(\cdot)$ is Legendre-Fenchel transform of $\psi(\cdot)$,
\[
\psi^{\star}(\epsilon)=\sup_{\lambda\in\mathbb{R}}\{\lambda\epsilon-\psi(\lambda)\}.
\]
Eq.(\ref{concention-ineq-01}) implies for any $\delta\in(0,1)$, the following holds with probability at least $1-\delta$, 
\[
\hat{\mu}_{a,t}+(\psi^{\star})^{-1}
\left(
\dfrac{1}{N_{a,t}}\log\dfrac{1}{\delta}
\right)
>\mu_a.
\]
\begin{algorithm}[h]
\caption{$(\alpha,\psi)\text{-}\mathtt{UCB}$ \citep{bubeck2012regret}}
\label{algo: alp-psai-ucb1}
\begin{algorithmic}[1]
\STATE Play each arm once, $t\leftarrow K$;
\FOR{$t=K,\cdots , T$}
\STATE Play $a_t=\arg\max_{a\in[K]}\left(\hat{\mu}_{a,t}+(\psi^{\star})^{-1}\sqrt{\dfrac{\alpha \log t}{N_{a,t}}}\right)$
\ENDFOR
\end{algorithmic}
\end{algorithm}
\begin{theorem}[Regret Analysis of $(\alpha,\psi)\text{-}\mathtt{UCB}$]
\label{theo:regret-of-ucb1}
Assume the reward satisfies (\ref{def:sub-gauassian}), $\alpha>2$, then the regret of $(\alpha,\psi)\text{-}\mathtt{UCB}$ (Algorithm \ref{algo: alp-psai-ucb1}) is upper-bounded as follows
\[
R^{(\alpha,\psi)\text{-}\mathtt{UCB} }(T)\leq
\sum_{a\ne a^{\star}}
\left(
\dfrac{\alpha\Delta_a }{\psi^{\star}\left(\frac{1}{2}\Delta_a\right)}\log T+\dfrac{\alpha}{\alpha-1}
\right).
\]
\end{theorem}
\begin{proof}
See \cite[Chapter 2]{bubeck2012regret}.
\end{proof}

\subsection{UCB($\delta$) \citep{lattimore2020bandit}}
In this section, we extend the distribution of reward $X$ to be subgaussian, we formally define it as follows.

\begin{definition}[Subgaussianity]
A random variable $X$ is $\sigma$-subgaussian with the variance factor $\sigma$, if for
all $\lambda\in\mathbb{R}^{1}$, it holds that \[\mathbb{E}[\exp\left\{\lambda (X-\mathbb{E}[X])\right\}] \leq\exp\left(\frac{1}{2}\lambda^2\sigma^2\right).\]
\end{definition}


\begin{example}[Bernoulli Distribution]
\label{example-1}
Let $X\sim\mathcal{B}(\mu)$, where $\mathcal{B}(\mu)$ is Bernoulli distribution with $\mathbb{P}(X=1)=\mu$ and $\mathbb{P}(X=0)=1-\mu$.
Then, $X$ is $\frac{1}{2}$-subgaussian.
For its proof, see \emph{\url{http://blog.wouterkoolen.info/BernoulliSubGaussian/post.html}}.
\end{example}



\begin{example}[Gaussian Distribution]
\label{example-2}
Let $X\sim\mathcal{N}(\mu,\sigma^2)$, where $\mathcal{N}(\mu,\sigma^2)$ is Gaussian distribution with expectation $\mu$ and standard deviation $\sigma$. 
Then, $X$ is $\sigma$-subgaussian. For its proof, please see \emph{\url{https://www.stat.berkeley.edu/~mjwain/stat210b/Chap2_TailBounds_Jan22_2015.pdf}}.
\end{example}




\begin{proposition}
\label{pro-hoeffding-iid}
Assume that $\{X_i\}_{i=1}^{n}$ are i.i.d, $\sigma$-subgaussian random variables with the expectation $\mu$. Let $\hat{\mu}_{n}=\frac{1}{n}\sum_{i=1}^{n}X_i$, then for any $\epsilon>0$, 
\begin{flalign}
\label{app-a-lemma}
\mathbb{P}\left(\left|\hat{\mu}_{n}-\mu\right|\ge \epsilon\right)\leq \exp\left\{-\dfrac{n\epsilon^2}{2\sigma^{2}}\right\}.
\end{flalign}
\end{proposition}
For the proof of Proposition \ref{pro-hoeffding-iid}, please refer to Corollary 5.5 in \citep{lattimore2020bandit}.
Furthermore, Proposition \ref{pro-hoeffding-iid} implies for any $\delta\in(0,1)$, the following holds with probability at least $1-\delta$, 
\begin{flalign}
\mu\leq \hat{\mu}_{n}+\sqrt{\dfrac{2\delta^2}{n}\log\frac{1}{\delta}},~~~~\mu\ge \hat{\mu}_{n}-\sqrt{\dfrac{2\delta^2}{n}\log\dfrac{1}{\delta}}.
\end{flalign}












==> preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}
In this section, we briefly review the basics of unimodal bandits and Thompson sampling.


We consider the MAB (stochastic multi-armed bandit) problem with $K$ arms.
At each round $t\in\mathbb{N}$, the decision maker pulls an arm $a\in[K]=:\{1,2,\cdots,K\}$, 
then it receives a random reward $X_{a,t}$ according to an unknown (but fixed) distribution $\nu_{a}$ that has an expectation $\mu_{a}=\mathbb{E}[X_{a,t}]$.
The random reward of each arm is independent identically distributed, 
and it is independent of the plays of other arms.
We assume that there is a unique optimal arm $a^{\star}$ satisfies $\mu^{\star}=:\mu_{a^{\star}}=:\max_{a\in[K]}\mu_{a}.$
We use $\Delta_a =: \mu^{\star}-\mu_a$ to denote the gap between the mean of the arm $a^{\star}$ and arm $a$.


\subsection{Unimodal Structure}

In this paper, we focus on the \emph{unimodal} bandit (U-MAB), where the expected reward function is monotonic over a partial order set of arms, 
which is an important class of bandit problems that have been studied by \cite{yu2011unimodal,combes2014unimodal_a}.
We use $\mathcal{G}=(\mathcal{V},\mathcal{E})$ to denote an undirected graph, where $\mathcal{V}=[K]$ denotes the vertices that are corresponding to arms, and the edges of the graph $\mathcal{G}$ characterize a partial order (initially unknown to the decision maker) among expected rewards.
We use $\nu=(\nu_{1},\cdots,\nu_{K})$ to denote the joint reward distribution, the partial order of $\mathcal{G}$ is unknown 
since $\nu$ is unknown.
We use $\mathcal{N}(a)$ to denote the neighborhood of arm $a$, specifically, $\mathcal{N}_a=\{a^{'}|(a,a^{'})\in\mathcal{E}\}$.
Without loss of generality, we assume $\mathcal{E}$ does not contain self-edges $(a, a)$ since it does not contribute to increasing paths \citep{trinh2020solving}.
The extended neighborhood of arm $a$ is denoted as follows $\mathcal{N}^{+}({a})=\mathcal{N}({a})\cup\{a\}$.



We make a precise expression of unimodal structure in the following Assumption \ref{ass-unimodal}.
\begin{assumption}[Unimodality\citep{combes2014unimodal_a}]
\label{ass-unimodal}
Let $\mathcal{G}=(\mathcal{V},\mathcal{E})$ denote an undirected graph.
For any sub-optimal arm $a\ne a^{\star}$, there exists a path 
$P=(a_1=a,a_2,\cdots,a_{m-1},a_m=a^{\star})$
(depending on the arm $a$), s,t.,
%there exists a path $p=(a_1 =k,\cdots, a_mk⋆)$ of length m (depending on k) such that for all i = 1, . . . , m − 1, (ki,ki+1) ∈ E and μki < μki+1 .
%The expected reward function is unimodal along each path $P=(a_1,\cdots,a_m)$ that contains $a^{\star}$,
%such that
\[\mu_a=\mu_{a_1}<\mu_{a_2}<\cdots<\mu_{a_{m-1}}<\mu_{a_m}=\mu_{a^{\star}},\]
where each $(a_{i},a_{i+1})\in\mathcal{E},1\leq i\leq m-1$.
\end{assumption}

The above assumption of unimodality is quite general, and it includes a special case: the classical unimodal function (where $\mathcal{G}$ is just a line). 




\subsection{Regret}
For the standard MAB problem, we use the loss of all generated rewards to measure the performance of a policy $\pi$.
Let $\mathcal{A}=\{ a_{t}\}_{t=1}^{T}$ be an action sequence that is generated by $\pi$.
The regret of the policy $\pi$ is defined as 
\begin{flalign}
\label{def:regret}
R^{\pi}(T)=\mathbb{E}\left[\sum_{t=1}^{T}(\mu^{\star}-X_{a_t,t})\right]=\sum_{a\ne a^\star}\Delta_a\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{a_{t}=a\}\right],
\end{flalign}
where the expectation $\mathbb{E}[\cdot]$ is taken with respect to the measure on outcomes induced by the interaction of the policy $\pi$ and the joint reward distribution $\nu$.

Now, we present the lower bound regret $R^{\pi}(T)$ of unimodal bandit problem.
Without loss of generality, we consider the uniformly good policy \cite{lai1985asymptotically}, i.e., $R^{\pi}(T)=o(T^{a})$, for some $a>0$.
Uniformly good policy always exist; for example, $\mathtt{UCB}$ (upper confidence bound, \cite{auer2002finite}) is uniformly good.



\begin{theorem}[\citep{combes2014unimodal_a}]
\label{the-1}
Let $\pi$ be a uniformly good policy.
Under Assumption \ref{ass-unimodal},
for a given unimodal bandit $\mathcal{G}=(\mathcal{V},\mathcal{E})$, the following holds,
\begin{flalign}
\label{lower-bound}
\lim_{T\rightarrow\infty}\inf \dfrac{R^{\pi}(T)}{\log(T)}\ge\sum_{a\in \mathcal{N}({a^\star})}\dfrac{\mu^\star-\mu_a}{\mathbb{KL}(\mu_{a}|\mu^\star)},
\end{flalign}
where $\mathbb{KL}(\mu_{a}|\mu^\star)=\mu_{a}\log\dfrac{\mu_a}{\mu^\star}+(1-\mu_{a})\log\dfrac{1-\mu_a}{1-\mu^\star}$ is KL-divergence between Bernoulli distributions of respective means $\mu_a$ and $\mu^\star$.
\end{theorem}


\begin{remark}
\cite{lai1985asymptotically} have shown the lower bound regret of standard MAB (but without unimodal structure) as follows,
\begin{flalign}
\label{lower-bound-lai1985}
\lim_{T\rightarrow\infty}\inf \dfrac{R^{\pi}(T)}{\log(T)}\ge\sum_{a\in [K]}\dfrac{\mu^{\star}-\mu_a}{\mathbb{KL}(\mu_{a}|\mu^\star)}.
\end{flalign}
The lower bound regret (\ref{lower-bound}) is very similar to standard MAB shown in (\ref{lower-bound-lai1985}), i.e., the regrets scale at least logarithmically with time.
However, since $\mathcal{G}=(\mathcal{V},\mathcal{E})$ equips an unimodal structure, the lower bound regret of (\ref{lower-bound}) improves the performance of standard MAB (\ref{lower-bound-lai1985}) significantly: 
the lower bound regret (\ref{lower-bound}) does not depend on the size of entire decision space $[K]$, and it is only controlled by the neighborhood of the optimal arm $a^{\star}$, i.e., the set $\mathcal{N}({a^{\star}})$.
We think it is not a surprising result, but it is natural:
due to the particularity of the additional unimodal structure, which makes it possible to design an algorithm with a better performance if we utilize the unimodal structure properly.
\end{remark}





\begin{algorithm}[t]
\caption{Thompson Sampling}
\label{alg:BernoulliTS}
\begin{algorithmic}[1]
\FOR{$t=1,2,\cdots $}
%\STATE \textcolor{blue}{\#sample model:}
\FOR{$a=1, \cdots, K$}
\STATE Sample $\hat{\theta}_{a,t} \sim \text{Beta}(\alpha_a, \beta_a)$
\ENDFOR \\
\STATE \textcolor{blue}{$\texttt{\#select and play action:}$}
\STATE $a_t \leftarrow \arg\max_{a\in [K]} \hat{\theta}_{a,t}$
\STATE Pull  $a_t$ and observe reward $X_{a_t,t}$
\STATE $(\alpha_{a_t}, \beta_{a_t}) \leftarrow  (\alpha_{a_t}, \beta_{a_t})+(X_{a_t,t}, 1-X_{a_t,t})$
\ENDFOR
\end{algorithmic}
\end{algorithm}



\subsection{Thompson Sampling}
Thompson Sampling \citep{thompson1933likelihood} is a Bayesian approach to make decisions according to its posterior probability. 
In this section, we only briefly present Thompson Sampling for Bernoulli rewards bandits with Beta prior, where the rewards of each arm $a$ are sampled from Bernoulli distribution $\mathcal{B}(\mu_a)$, i.e., $X_{a,t}\sim\mathcal{B}(\mu_a)$, and $X_{a,t}\in \{0,1\}$.
When played, an action $a\in[K]$ produces a reward of $\mathtt{one}$ with probability $\theta_a$, and a reward of $\mathtt{zero}$ with probability $1-\theta_a$.
Each $\theta_a$ can be interpreted as an action's success probability or mean reward.  
The mean reward vector $\bm{\theta}=(\theta_1,...,\theta_K)$ is unknown, but fixed over time.  
Initially, we assume the expected reward $\mu_a$ of each arm $a$ has the prior distribution Beta$(1, 1)$ that is the uniform distribution over $[0, 1]$.
Thus each arm $a\in[K]$ equips with the same probability to be played initially.
At round $t$, the posterior distribution of each action $a$ is also a Beta distribution Beta$(\alpha_a, \beta_a)$ with parameters
that can be updated according to a simple rule:
\begin{flalign}
\nonumber
 (\alpha_a, \beta_a) &\leftarrow
 \begin{cases}
     (\alpha_a, \beta_a)    & \text{if } a \neq a_t \\
     (\alpha_a, \beta_a)+(X_{a_t,t}, 1-X_{a_t,t})      & \text{if } a =a_t.
 \end{cases}
 \end{flalign}
 We provide the complete scheme in Algorithm \ref{alg:BernoulliTS}.
\cite{agrawal2013further} have shown that Thompson Sampling asymptotically matches its lower bound (\ref{lower-bound-lai1985}), see the next Theorem \ref{app-a-optimal-regret}.
 
 
\begin{theorem}[\cite{agrawal2013further}]
\label{app-a-optimal-regret}
For the $K$-armed stochastic bandit problem, Thompson Sampling using Beta priors has expected regret
\[
R(T)\leq(1+\epsilon)  \sum_{a\ne a^\star} \dfrac{\mu^\star-\mu_a}{\mathbb{KL}(\mu_a|\mu^\star)}\log T +\mathcal{O}\left(\frac{K}{\epsilon ^2}\right).
\]
\end{theorem}






\section{Asymptotically Optimal Unimodal Bandit Algorithms: An Overview}
\label{Existing-work}


Pioneer works of unimodal bandit algorithms can be traced back to \citep{kleinberg2004nearly,kleinberg2008multi,cope2009regret,yu2011unimodal,combes2014unimodal_b}, but they are all not asymptotically optimal.
In this section,
we mainly review asymptotically optimal unimodal bandit algorithms: forced-exploitation based approaches, e.g., $\texttt{OSUB}$ \citep{combes2014unimodal_a}, $\texttt{UTS}$ \citep{paladino2017unimodal};
forced-exploitation free based approaches, e.g., $\texttt{KLUCB}$-$\texttt{UB}$, $\texttt{IMED}$-$\texttt{UB}$  \cite{saber2020forced}.


\textbf{Notations}.
Let $N_{a,t}=\sum_{j=1}^{t}\mathbb{I}\{{a_j=a}\}$ be the number of times arm $a$ has been played after $t$ rounds, where $\mathbb{I}\{\cdot\}$ is the indicator function, i.e., $\mathbb{I}\{{E}\}=1$ if ${E}$ occurs; otherwise $\mathbb{I}\{{E}\}=0$.
Let 
\[\hat{\mu}_{a,t}=\dfrac{\sum_{j=1}^{t}\mathbb{I}\{{a_j=a}\}X_{a,j}}{N_{a,t}},~~
\hat{\mu}^{\star}_{t}=\max_{a\in[K]}\hat{\mu}_{a,t}
\]
be the empirical reward mean received from arm $a$ at round $t$ and current best mean.
The \emph{leader} $L_{t}$ is the arm that have the maximal empirical mean of rewards at current round $t$: \[L_t=\arg\max_{a\in [K]}\{\hat{\mu}_{a,t}\},\] and $n_{a,t}=\sum_{j=1}^{t}\mathbb{I}\{L_j=a\}$ is the number of times that arm $a$ has been chosen as the leader at the end of round $t$.












\subsection{Forced-Exploitation Algorithms}


To solve the U-MAB problem, \cite{combes2014unimodal_a} introduce a forced-exploitation mechanism that forces the player to pull the current leader at a fixed frequency.
Later,  \cite{paladino2017unimodal,trinh2020solving} extend such a forced-exploitation mechanism to Thompson Sampling.
In this section, we briefly review those two typical algorithms.




$\textbf{OSUB}$.
 $\texttt{OSUB}$ \cite{combes2014unimodal_a} is based on $\texttt{KL}$-$\texttt{UCB}$ \citep{garivier2011kl,cappe2013kullback} 
 that uses KL-divergence upper confidence bounds to define an index for each arm. 
Exploration on the neighborhood of the current leader is a novel idea of $\texttt{OSUB}$.
Concretely, 
$\texttt{OSUB}$ pulls an action according to the following rule:
\begin{flalign}
\label{osub-action-algo}
a_t=
\begin{cases}
L_t,      & \text{if}~\dfrac{n_{L_t,t}-1}{\gamma+1}\in\mathbb{N}  \\
\arg\max_{a\in \mathcal{N}^{+}({L_t})}
F_{a,t-1}
        & \text{otherwise,}\\
\end{cases}
\end{flalign}
where \[F_{a,t-1}=\sup \left\{\nu\ge\hat{\mu}_{a,t}:N_{a,t}\mathbb{KL}(\hat{\mu}_{a,t-1}|\nu)\leq {f(n_{L_t,t})} \right\},\] $f(\cdot)=\log (\cdot)+ \log \log (\cdot)$, 
and $\gamma$ is a factor that forces the player to pull the current leader at a fixed frequency.
\cite{combes2014unimodal_a} suggest to set $\gamma$ to be the maximal degree of nodes in $\mathcal{G}$.
Although \cite{combes2014unimodal_a} show that $\texttt{OSUB}$ is an asymptotically optimal algorithm, it's too expensive to calculate $F_{a,t-1}$. 
For example, \cite{filippi2010optimism} have applied Newton's method to solve $F_{a,t-1}$, which is impractical for complex decision-making tasks since it requires a very high computational complexity.




$\textbf{UTS}$.
\cite{paladino2017unimodal} inherit the forced-exploitation mechanism from \cite{combes2014unimodal_a}, and design a Thompson Sampling based algorithm called $\texttt{UTS}$ to solve the unimodal bandit problem.
Concretely, instead of playing an action according to $\texttt{Line}~\texttt{6}$ of Algorithm \ref{alg:BernoulliTS}, 
$\texttt{UTS}$ pulls an arm as follows,
\begin{flalign}
\label{uts-update-01}
a_t=
\begin{cases}
L_t,      & \text{if}~\dfrac{n_{L_t,t}}{\gamma}\in\mathbb{N}  \\
\arg\max_{a\in \mathcal{N}^{+}({L_t})}\hat{\theta}_{a,t}
        & \text{otherwise,}\\
\end{cases}
\end{flalign}
where $\gamma=|\mathcal{N}^{+}({L_t})|$, the procedure that generates $\hat{\theta}_{a,t}$ is as the same estimate as standard Thompson Sampling i.e., Algorithm \ref{alg:BernoulliTS}, and $|\cdot|$ is the cardinality operator.
\cite{paladino2017unimodal} have shown that $\texttt{UTS}$ is also an asymptotically optimal algorithm.
Recently, \cite{trinh2020solving} propose $\texttt{UTS}$ resembles (\ref{uts-update-01}), but they focus on solving an instance of unimodal bandit problem: \emph{rank-one bandit} problem \citep{katariya2017bernoulli}.
Particularly, \cite{trinh2020solving} refine some key steps of proof in \cite{paladino2017unimodal}, and  provide a precise analysis of $\texttt{UTS}$ to corroborate its good empirical performance for rank-one bandits.



\begin{remark}
\label{discuss: forced-exploitation mechanism}
Both $\texttt{UTS}$ and $\texttt{OSUB}$ depend heavily on the forced-exploitation mechanism.
It is still a very complicating and confusing problem that  $\texttt{UTS}$ and $\texttt{OSUB}$ performs at what a frequency can achieve the best performance.
Although \cite{trinh2020solving} have provided some insights on the calibration of the leader exploration parameter to get a better performance via certain experiments, their empirical method seems to tune the frequency factor $\gamma$ manually,
which is very inefficient and cumbersome for complex sequence decision making tasks.
More importantly, as stated by \cite{saber2020forced}, it is still under debate 
whether or not those forcing mechanisms are desirable features in the community.
\end{remark}



\subsection{Forced-Exploitation Free Algorithms}

Recently, \cite{saber2020forced} firstly abandon the forced-exploitation mechanism and propose two forced-exploitation free strategies: $\texttt{IMED}$-$\texttt{UB}$ and $\texttt{KLUCB}$-$\texttt{UB}$.


\textbf{IMDE-UB}.
Concretely, $\texttt{IMED}$-$\texttt{UB}$ adapts the $\texttt{IMED}$ (indexed minimum empirical divergence) strategy \citep{honda2015non}, and it plays an action as follows,
\begin{flalign}
\label{imde-ub}
a_t\leftarrow\arg\min_{a\in\mathcal{N}^{+}({L_t})}
\left\{
N_{a,t}\mathbb{KL}(\hat{\mu}_{a,t}|\hat{\mu}^{\star}_{t})+\log(N_{a,t})
\right\}.
\end{flalign}
The index in (\ref{imde-ub}) can be seen as a transportation cost for moving a
sub-optimal arm to an optimal one plus an exploration term: the logarithm of the numbers of pulls.
When an optimal arm is considered, the transportation cost is null and there is only the exploration
part. 

\textbf{KLUCB-UB}.
Furthermore, \cite{saber2020forced} refine the scheme of $\texttt{OSUB}$ and propose $\texttt{KLUCB}$-$\texttt{UB}$ algorithm that pulls an arm as follows,
\begin{flalign}
\label{kl-ucb-ub}
a_t=\arg\max_{a\in \mathcal{N}^{+}({L_t})}G_{a,t-1}
\end{flalign}
where $G_{a,t-1}=\sup \left\{\nu\ge\hat{\mu}_{a,t}:N_{a,t}\mathbb{KL}(\hat{\mu}_{a,t-1}|\nu)\leq {g_t)} \right\}$
$g_t=\log (n_{{L_t},t})-\log (N_{a,t})$.


\cite{saber2020forced} have shown the asymptotic optimality of $\texttt{IMED}$-$\texttt{UB}$/$\texttt{KLUCB}$-$\texttt{UB}$.
It is an open problem that whether the asymptotic optimality can occur for forced-exploitation free $\texttt{UTS}$, in the next section, we give a positive answer.



\section{Forced-Exploitation Free Unimodal Thompson Sampling}
\label{sec:ts-ub-bernoulli-reward}

In this section, we extend Thompson Sampling to solve the U-MAB problem and propose $\texttt{FEF}$-$\texttt{UTS}$ (forced-exploitation free unimodal Thompson Sampling).
We show $\texttt{FEF}$-$\texttt{UTS}$ shares the same asymptotically optimal regret as $\texttt{OSUB}$ and $\texttt{UTS}$.
Finally, we provide a technical overview of proof and present the main challenges to achieving the asymptotic optimality of $\texttt{FEF}$-$\texttt{UTS}$.




\subsection{Algorithm}

We provide the pseudo-code of $\texttt{FEF}$-$\texttt{UTS}$ for Bernoulli rewards in Algorithm \ref{alg:TS-UB}.
The main difference between $\texttt{UTS}$ (\ref{uts-update-01}) and $\texttt{FEF}$-$\texttt{UTS}$ is that 
$\texttt{FEF}$-$\texttt{UTS}$ does not use any forced exploitation factor $\gamma$ that appears in $\texttt{UTS}$ (\ref{uts-update-01}), where it uses  $\gamma$ to control the frequency of playing the current leader.
Although $\texttt{FEF}$-$\texttt{UTS}$ playing the action resembles the standard Thompson Sampling, it is worth noticing the following two aspects.


\textbf{Exploration}.~Our $\texttt{FEF}$-$\texttt{UTS}$ uses Beta distribution to explore the potential arms that may yield high rewards in the future.
To take advantage of the additional unimodal structure, $\texttt{FEF}$-$\texttt{UTS}$ explores the arms only come from $\mathcal{N}^{+}({L_t})$, i.e., the neighborhood of the current leader.
Now, we provide some intuitions behind the idea of local neighborhood exploration.
After adequate explorations, the current leader should approximate the optimal action.
We believe the current leader's neighborhood should contain all the ``good" actions due to the unimodal structure.
Thus, it is a natural idea to explore arms in the neighborhood of the current leader.
While Thompson Sampling explores arms from the entire decision space $[K]$, i.e., $\texttt{Line}$ $\texttt{6}$ in Algorithm \ref{alg:BernoulliTS}.
This slight change makes a fundamental difference of regret between Thompson Sampling and $\texttt{FEF}$-$\texttt{UTS}$. To clarify this difference, we provide a deep discussion in Remark \ref{remark-1}.




\textbf{Exploitation}.~To utilize the current information of each arm, $\texttt{FEF}$-$\texttt{UTS}$ tries to play the current leader $L_{t}$ often.
Thus, for each round $t$, $\texttt{FEF}$-$\texttt{UTS}$ plays an arm in the neighborhood of $L_{t}$ (see $\texttt{Line~10}$, Algorithm \ref{alg:TS-UB}).

\begin{remark}[Comparison with $\texttt{KLUCB}$-$\texttt{UB}$ and $\texttt{IMED}$-$\texttt{UB}$]
Although Saber et.al. \cite{saber2020forced} firstly introduce the forced-exploitation free mechanism to U-MAB and propose $\texttt{KLUCB}$-$\texttt{UB}$ and $\texttt{IMED}$-$\texttt{UB}$, which are frequentist approaches that contrast with our Bayesian approach $\texttt{FEF}$-$\texttt{UTS}$.
Concretely, $\texttt{KLUCB}$-$\texttt{UB}$ (\ref{kl-ucb-ub}) and $\texttt{IMED}$-$\texttt{UB}$ (\ref{imde-ub}) pull an arm according to an index that is defined by KL-divergence, while $\texttt{FEF}$-$\texttt{UTS}$ makes a decision according to the posterior distribution.
Notably,  likes $\texttt{OSUB}$ and $\texttt{KLUCB}$, $\texttt{KLUCB}$-$\texttt{UB}$ is involved to an intractable optimization problem that requires a very high computational complexity, which makes $\texttt{KLUCB}$-$\texttt{UB}$ difficult to search the optimal action efficiently for complex decision-making tasks.
Our $\texttt{FEF}$-$\texttt{UTS}$ does not require to solve any optimization problems, and it keeps the advantage of simplicity for implementation.
\end{remark}


\begin{algorithm}[t]
\caption{Forced-Exploitation Free Unimodal Thompson Sampling (FEF-UTS)} 
\label{alg:TS-UB}
\begin{algorithmic}[1]
\STATE \textbf{Input:} graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$ with unimodal structure; 
\STATE \textbf{Initizlize:} $\{\alpha_{a}=1,\beta_{a}=1,\hat{\mu}_{a,t=0}=0\}_{a=1}^K$
\FOR{$t=1,2,\ldots $}
\vspace{3pt}
\STATE{\color{blue}{$\texttt{\# search the leader globally:}$}}
\STATE $L_t\leftarrow\arg\max_{a\in [K]}\{\hat{\mu}_{a,t-1}\}$
%\STATE {\color{blue}{ \# sample the model:}}
\FOR{$a=1, \cdots, K$}
\STATE Sample $\hat{\theta}_{a,t} \sim\text{Beta}(\alpha_{a},\beta_{a})$
\ENDFOR
%\vspace{3pt}
    %\STATE Sample $\hat{\theta}_{a,t} \sim\text{Beta}(\alpha_{a},\beta_{a})$
    \vspace{3pt}
     \STATE{\color{blue}{$\texttt{\# play an action locally :}$}}
     %\vspace{3pt}
    \STATE $a_t \leftarrow \arg\max_{a \in \mathcal{N}^{+}(L_t)} \hat{\theta}_{a,t}$
% \ENDIF
\vspace{3pt}
\STATE Pull $a_t$ and observe reward $X_{a_t,t}$ 
\vspace{3pt}
\STATE Compute empirical reward $\hat{\mu}_{a,t}$, $a\in [K]$
\vspace{3pt}
\STATE{\color{blue}{$ \texttt{\# update Beta distribution:}$}}
\STATE $(\alpha_{a_t}, \beta_{a_t}) \leftarrow  (\alpha_{a_t}, \beta_{a_t})+(X_{a_t,t}, 1-X_{a_t,t})$
\vspace{3pt}
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Asymptotic Optimality}

\begin{theorem}
\label{them:regret-TS-UB}
Under Assumption \ref{ass-unimodal}, for any positive $\epsilon$, $\texttt{FEF}$-$\texttt{UTS}$ (Algorithm \ref{alg:TS-UB}) has a regret as follow,
\begin{flalign}
\label{regret-algo2}
R(T)&\leq(1+\epsilon)\sum_{a\in\mathcal{N}({a^\star})} \dfrac{\mu_{\star}-\mu_a}{\mathbb{KL}(\mu_a|\mu^\star)} \log T+\mathcal{O}\left(\frac{|{\mathcal{N}({a^\star})}|}{\epsilon ^2}\right)
+\sum_{a\ne a^\star}\left(\dfrac{4}{\Delta_a^2}+\dfrac{{2\sqrt{\pi}}}{\Delta_a}+C+D\right),
\end{flalign}
where $C$ and $D$ are two positive scalars that are defined in Appendix \ref{app-b-proof-1}.
\end{theorem}
From the details of proof in Appendix \ref{app-b-proof-1}, we know the regret (\ref{regret-algo2}) can be interpreted by two distinct cases, 
when the sub-optimal arm $a(\ne a^\star)$ is leader, and when the optimal arm $a^\star$ is leader:


\textbf{Case(i)}.When the sub-optimal $a~(\ne a^\star)$ is selected to be leader, the regret is upper-bounded by a constant
\[
\sum_{a\ne a^\star}\left(\dfrac{4}{\Delta^2_a}+\dfrac{{2\sqrt{\pi}}}{\Delta_a}+C+D\right).\
\]
To achieve this result, we provide a novel analysis that is significantly different from the previous unimodal bandit algorithms $\texttt{OSUB}$ \cite{combes2014unimodal_a} and $\texttt{UTS}$ \cite{paladino2017unimodal,trinh2020solving}.









\textbf{Case(ii)}.When the optimal arm $a^\star$ is selected to be leader, the regret is upper-bounded as follows,
\[
(1+\epsilon)\sum_{a\in\mathcal{N}({a^\star})} \dfrac{\mu^{\star}-\mu_a}{\mathbb{KL}(\mu_a|\mu^\star)}\log T+\mathcal{O}\left(\dfrac{|{\mathcal{N}({a^\star})}|}{\epsilon ^2}\right),
\]
which resembles the upper-bound regret of Thompson Sampling \cite{agrawal2013further}, we have presented it in Lemma \ref{app-a-optimal-regret} in Appendix \ref{sec:app-ts}.
Since we consider the unimodal structure, our result holds on the set ${\mathcal{N}({a^\star})}$ exactly, we have formulated this result in Proposition \ref{pro:bound-regret-1}, see Section \ref{Proof-Overview}.




The term $ \sum_{a\in{\mathcal{N}({a^\star})}} \dfrac{\mu^{\star}-\mu_a}{\mathbb{KL}(\mu_a|\mu^\star)}\log T$ in Eq.(\ref{regret-algo2}) is the optimal asymptotic regret that matches the lower bound in Theorem \ref{lower-bound}, which is also determined by the neighborhood of optimal arm $a^\star$: $\mathcal{N}(a^{\star})$.
For Eq.(\ref{regret-algo2}), $\epsilon$ is often chosen to be a small positive constant.
However, we notice that if we choose a too small $\epsilon$, then the term $\mathcal{O}\left(\dfrac{|{\mathcal{N}({a^\star})}|}{\epsilon ^2}\right)$ can be very large.
The next Corollary \ref{optimalty-1} provides a sufficient condition of $\epsilon$ that guarantees the asymptotic optimality of $\texttt{FEF}$-$\texttt{UTS}$ algorithm.
%and it shows that the proposed Algorithm \ref{them:regret-TS-UB} matches the lower bound in Theorem \ref{the-1}.
\begin{corollary}[Asymptotic Optimality]
\label{optimalty-1} 
Under Assumption \ref{ass-unimodal},
let $\epsilon\in\left(\frac{1}{\sqrt{\log T}},1\right)$, e.g., $\epsilon=(\log T)^{-\frac{1}{3}}$, $\texttt{FEF}$-$\texttt{UTS}$ (Algorithm \ref{alg:TS-UB}) has a regret as follow,
\begin{flalign}
\label{ts-ub-upperbound-1}
\lim_{T\rightarrow\infty}\dfrac{R(T)}{\log(T)}\leq\sum_{a\in {\mathcal{N}({a^\star})}}\dfrac{\mu^{\star}-\mu_a}{\mathbb{KL}(\mu_{a}|\mu^\star)}.
\end{flalign}
\end{corollary}
\begin{proof}
See Appendix \ref{app-b-proof-2}.
\end{proof}









\begin{remark}
[Comparison with Forced-Exploitation Algorithms]
\label{remark-comparison-uts-osub}
Comparing with $\texttt{OSUB}$ (\ref{osub-action-algo}) and $\texttt{UTS}$ (\ref{uts-update-01}), the forced-exploitation factor $\gamma$ never appears in $\texttt{FEF}$-$\texttt{UTS}$.
%According to Theorem 5 of \cite{trinh2020solving}, our $\texttt{FEF}$-$\texttt{UTS}$ shares the same order of regret of \cite{trinh2020solving},
% but $\texttt{FEF}$-$\texttt{UTS}$ is simpler since it does not need to tune $\gamma$.
\cite{combes2014unimodal_a,paladino2017unimodal} have shown that the regret of $\texttt{UTS}$ and $\texttt{OSUB}$ are all upper-bounded as follows,
\begin{flalign}
\label{UTS-rw}
(1+\epsilon) \sum_{a\in{\mathcal{N}({a^\star})}} \dfrac{\mu^{\star}-\mu_a}{\mathbb{KL}(\mu_a|\mu^\star)}  \left(\log T +\log (\log T)\right)+C_1,
\end{flalign}
where $C_1$ is a fixed constant. 
For a given $\epsilon$, if the horizon $T$ is very large, 
the upper bound of $\texttt{FEF}$-$\texttt{UTS}$ (\ref{regret-algo2}) is never worse than (\ref{UTS-rw}),
Thus, the proposed $\texttt{FEF}$-$\texttt{UTS}$ is more simpler for implementation but more effective than the above two unimodal bandit algorithms.
\end{remark}
\begin{remark}[Comparison with Standard Thompson Sampling]
\label{remark-1}
Notably, exploration within the neighborhood of its current leader is the essential difference between $\texttt{FEF}$-$\texttt{UTS}$ and Thompson Sampling.
\cite{agrawal2013further} have shown that Thompson Sampling asymptotically matches its lower bound (\ref{lower-bound-lai1985}),  which is determined by the entire decision space $[K]$.
For a given unimodal bandit, Eq.(\ref{ts-ub-upperbound-1}) reveals that the asymptotical regret of $\texttt{FEF}$-$\texttt{UTS}$ only depends on the neighborhood of the optimal arm $a^{\star}$, 
thus the regret of $\texttt{FEF}$-$\texttt{UTS}$ is never worse than Thompson Sampling.
That also implies exploration within the neighborhood of its current leader could be more efficient than exploring on the entire decision space $[K]$ when we consider solving unimodal bandit problems.
\end{remark}



\section{Proof Overview of Theorem \ref{}}
\label{Proof-Overview}



We start by distinguishing the times when the leader is the optimal arm $a^{\star}$ and when it is not:
\begin{flalign}
\label{decopmsi-regret}
R(T)&= R_1(T)+R_2(T),
\end{flalign}
where
\begin{flalign}
\nonumber
R_{1}(T)=\sum_{a\ne a^\star}\Delta_a\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{a_{t}=a,L_t=a^{\star}\}\right],
R_{2}(T)=\sum_{a\ne a^\star}\Delta_a\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{a_{t}=a,L_t=a(\ne a^{\star})\}\right],
\end{flalign}
i.e., $R_{1}(T)$ denotes regret if the leader is $a^{\star}$, otherwise the regret is $R_{2}(T)$.
In fact, it is easy to check the following equation,
\begin{flalign}
\label{app-a-2}
\mathbb{I}\{a_{t}=a\}=\mathbb{I}\{\underbrace{L_{t}=a^\star,a_t=a}_{(\text{i})}\}+\mathbb{I}\{\underbrace{L_{t}\ne a^\star,a_t=a}_{(\text{ii})}\},
\end{flalign}
where event $(\text{i})$ is the case when the best arm $a^\star$ is the leader, other case is the even $(\text{ii})$.
Taking Eq.(\ref{app-a-2}) into Eq.(\ref{def:regret}), we have
\begin{flalign}
%\label{app-a-3}
\nonumber
R(T)&=\underbrace{\sum_{a\ne a^\star}(\mu^\star-\mu_a)\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{L_{t}=a^\star,a_t=a\}\right]}_{=:R_1(T)}+\underbrace{\sum_{a\ne a^\star}(\mu^\star-\mu_a)\mathbb{E}\left[\sum_{t=1}^{T}\mathbb{I}\{L_{t}\ne a^\star,a_t=a\}\right]}_{=:R_2(T)},
\end{flalign}
thus Eq.(\ref{decopmsi-regret}) holds.
This result requires us to upper bound the terms $R_{1}(T)$ and $R_{2}(T)$ correspondingly.



\subsection{Bound $R_{1}(T)$: the case when the optimal action $a^{\star}$ chosen as leader}



To bound $R_{1}(T)$, we should notice that 
when $a^{\star}$ is the leader, 
the update rule of $\texttt{FEF}$-$\texttt{UTS}$ implies
the played arm $a$ necessarily belongs to the neighborhood of $a^{\star}$.
Thus, when $a^{\star}$ is the leader,  the proposed $\texttt{FEF}$-$\texttt{UTS}$ behaves as standard Thompson Sampling restricted on the set $\mathcal{N}^{+}(a^{\star})$.
Such an idea has be used for the regret analysis of $\texttt{OSUB}$ and $\texttt{UTS}$ by \cite{combes2014unimodal_a,paladino2017unimodal}, \cite{trinh2020solving} respectively.
Therefore, according to the same analysis by \citep{agrawal2013further} (we have presented in Theorem \ref{app-a-optimal-regret}), we achieve the upper bound regret of $R_{1}(T)$ in the next Proposition \ref{pro:bound-regret-1}.
\begin{proposition}
\label{pro:bound-regret-1}
Under Assumption \ref{ass-unimodal}, for any positive $\epsilon$, $T\ge1$, regret $R_{1}(T)$ is upper-bounded as follows,
\[
R_1(T)\leq
(1+\epsilon)\sum_{a\in{\mathcal{N}({a^\star})}} \frac{\mu^{\star}-\mu_a}{\mathbb{KL}(\mu_a|\mu^\star)}\log T+\mathcal{O}\left(\frac{|{\mathcal{N}({a^\star})}|}{\epsilon ^2}\right).\]
\end{proposition}







\subsection{Bound $R_{2}(T)$: the case when the sub-optimal action $a\ne a^{\star}$ chosen as leader}


The main challenge to show Theorem \ref{them:regret-TS-UB} is to 
get the upper boundedness of $R_{2}(T)$.
Firstly, we present the upper bound of $R_{2}(T)$ in the following Proposition \ref{pro:bound-regret-2}; then we present the main technique to proof Proposition \ref{pro:bound-regret-2}.

\begin{proposition}
\label{pro:bound-regret-2}
Let $D_a(x)=\mathbb{KL}(x|\mu_a)$ be short for KL-divergence between Bernoulli distributions,
\[c_a=
 \log\left(\frac{1}{e^{D_{a}(\mu^{\star}-\frac{\Delta_a}{4})}-1}\right)+D_{a}(\mu^{\star}-\frac{\Delta_a}{4}) e^{D_{a}(\mu^{\star}-\frac{\Delta_a}{4})}
\]
\[
 d_a=
 \log\left(\frac{1}{e^{D_{a}(|\mu_a-\frac{\Delta_a}{8}|)}-1}\right)+D_{a}(|\mu_a-\frac{\Delta_a}{8}|) e^{D_{a}(|\mu_a-\frac{\Delta_a}{8}|)}.
\]
Then, for any $\delta_1\in(0,{\mu_a +\frac{\Delta_a}{8}})$,
the regret $R_{2}(T)$ is upper-bounded as follows
\footnote
{
Notation $\Theta(\cdot)$: for any two functions $f(\cdot),g(\cdot)$, we denote $f(x) = \Theta(g(x))$ if there exists constants $a,b$ and $x_0$ such that for all $x \ge x_0$, $ag(x) \leq f(x) \leq bg(x).$
},
\begin{flalign}
\nonumber
R_{2}(T)
\leq&
\sum_{a\ne a^{\star}}
\Bigg(
\dfrac{1}{\mu_a+\frac{\Delta_a}{8}-\delta_1}
+
\dfrac{1}{\mathbb{KL}\left(\delta_1\Big|{\mu_a +\frac{\Delta_a}{8}}\right)}+
\Theta
\left(
\dfrac{2336+16c_a+64d_a}{\Delta^{2}_a}
\right)
+\dfrac{4}{\Delta^2_a}+\dfrac{2\sqrt{\pi}}{\Delta_a}
\Bigg).
%\\
%\nonumber
%=:&\sum_{a\ne a^{\star}}\left(\dfrac{4}{\Delta^2_a}+\dfrac{2\sqrt{\pi}}{\Delta_a}+C+D\right)
\end{flalign}
%where $C$ and $D$ are two positive scalars that are defined in Appendix \ref{app-b-proof-1}.
\end{proposition}
\begin{proof}
See Appendix \ref{app-sec:prop-02}.
\end{proof}


\begin{framed}
For convenience of reference, we list the key steps to prove Proposition \ref{pro:bound-regret-2} as follows,
\begin{flalign}
\nonumber
R_{2}(T)&\overset{\text{Lemma~\ref{lemma-5}}}\leq \sum_{a\ne a^\star}\mathbb{E}[n_{a,T}]\overset{\text{Lemma~\ref{app:lemma5-01}}}
\leq 
\underbrace{\text{Term~I~(\ref{app:lemma5-02})}}_{\text{Upper-bound~by~Lemma~\ref{lemma-7}}}
+
\underbrace{
\text{Term~II~(\ref{app:lemma5-02})}
}_{\text{Upper-bound~by~Lemma~\ref{lemma-8}}}.
\end{flalign}
\end{framed}
Lemma \ref{lemma-5} illustrates the upper bound of $R_{2}(T)$ is related to the expectation of choosing any given suboptimal arm $a$ as the leader, 
\begin{flalign}
R_{2}(T)\leq \sum_{a\ne a^\star}\mathbb{E}[n_{a,T}]=\sum_{a\ne a^\star}\sum_{t=1}^{T}\mathbb{P}\left(\hat{\mu}_{a,t}=\max_{i\in[K]}\hat{\mu}_{i,t}\right),
\end{flalign}
which has appeared in the previous works of U-MAB (e.g., \cite{combes2014unimodal_a,paladino2017unimodal,trinh2020solving}).





Since $L_t=a\ne a^\star$, i.e., we consider the case that the suboptimal arm $a$ is selected as a leader, then 
$\hat{\mu}_{a,t}\ge\hat{\mu}_{a^\star,t}.$
It is easy to check the following event occurs 
\begin{flalign}
\label{step:1-esti}
\{\hat{\mu}_{a,t}=\max_{i\in[K]}\hat{\mu}_{i,t}\}\subset\{\hat{\mu}_{a,t}\ge\hat{\mu}_{a^\star,t}\}.
\end{flalign}
Furthermore, according to (\ref{step:1-esti}), Lemma \ref{app:lemma5-01} shows
\begin{flalign}
\label{upper-bound-01}
R_{2}(T)\leq
\text{Term~I~(\ref{app:lemma5-02})}
+
\text{Term~II~(\ref{app:lemma5-02})},
\end{flalign}
where 
\begin{flalign}
\nonumber
\text{Term~I~(\ref{app:lemma5-02})}&=
\sum_{a\ne a^\star}\sum_{t=1}^{T}\mathbb{P}\left(\hat{\mu}_{a,t}-\mu_a\ge \frac{\Delta_a}{2}\right)\\
\nonumber
\text{Term~II~(\ref{app:lemma5-02})}&=\sum_{a\ne a^\star}\sum_{t=1}^{T}\mathbb{P}\left(\mu^\star- \hat{\mu}_{a^\star,t}\ge\frac{\Delta_a}{2}\right).
\end{flalign}
Eq.(\ref{upper-bound-01}) implies we need to \text{Term~I~(\ref{app:lemma5-02})} and \text{Term~II~(\ref{app:lemma5-02})}.

To bound \text{Term~I~(\ref{app:lemma5-02})}, we
control their expected cardinalities using concentration inequalities, which is relatively easy and we have provide the details in Lemma \ref{lemma-7}.



Bounding \text{Term~II~(\ref{app:lemma5-02})} is more involved. Let $\vartheta^{\star}_{t}=\max_{a\in\mathcal{N}^{+}(L_t)}\{\hat{\theta}_{a,t}\}$ be the maximal posterior sample restricted on the neighbor of current leader $L_t$, furthermore,
\begin{flalign}
\nonumber
&\mathbb{P}\left(\mu^\star- \hat{\mu}_{a^\star,t}\ge\frac{\Delta_a}{2}\right)\\
\label{app-tem-imsec-01}
\leq&\mathbb{P}\left(\mu^\star-\vartheta^{\star}_{t}\ge\frac{\Delta_a}{4}\right)+
\mathbb{P}\left(\vartheta^{\star}_{t}-\hat{\mu}_{a^\star,t}\ge\frac{\Delta_a}{4}\right).
\end{flalign}
Since $\vartheta^{\star}_{t}$ is sampled from Beta distribution,
we need the transformation between Beta and Binomial distribution: $F^{\text{Beta}}_{a,b}(y)=1-F^{\text{B}}_{a+b-1,y}(a-1)$ to bound the \text{Term~II~(\ref{app:lemma5-02})}, where $F^{\text{Beta}}_{a,b}$ denotes the c.d.f of a Beta distribution with parameters $a$ and $b$, $F_{n,p}(k)$ denotes the c.d.f of a Binomial distribution with parameters $n$ and $p$.
We provide the complete proof in Lemma \ref{lemma-8}.

























Finally, taking the bounds in Proposition \ref{pro:bound-regret-1}-\ref{pro:bound-regret-2} together, we achieve the upper-bound regret of $\texttt{FEF}$-$\texttt{UTS}$.





















\section{ Conclusion}

In this paper, we introduce Thompson Sampling to solve unimodal bandits problem and propose $\texttt{FEF}$-$\texttt{UTS}$.
$\texttt{FEF}$-$\texttt{UTS}$ does not consider the forced-exploitation mechanism.
To exploit the unimodal structure better, 
at each step, instead of exploration from the entire decision space,
$\texttt{FEF}$-$\texttt{UTS}$ makes decisions only in the neighborhood of the arm that has the highest empirical mean reward.
We theoretically prove the asymptotic optimality of $\texttt{FEF}$-$\texttt{UTS}$.
Finally, we use experiments to demonstrate the effectiveness of the proposed algorithm, results show that $\texttt{FEF}$-$\texttt{UTS}$ performs better than extensive state-of-the-art algorithms.

 

